Over-the-air Function Computation in Sensor Networks

Many sensor applications are interested in computing a function over measurements (e.g., sum, average, max) as opposed to collecting all sensor data. Today, such data aggregation is done in a cluster-head. Sensor nodes transmit their values sequentially to a cluster-head node, which calculates the aggregation function and forwards it to the base station. In contrast, this paper explores the possibility of computing a desired function over the air. We devise a solution that enables sensors to transmit coherently over the wireless medium so that the cluster-head directly receives the value of the desired function. We present analysis and preliminary results that demonstrate that such a design yield a large improvement in network throughput.

==> revision.tex <==
\newcommand{\Revision}{}

